Competition Dynamics in the Meme Ecosystem

The creation and sharing of memes is a common modality of online social interactions. The goal of the present work is to better understand the collective dynamics of memes in this accelerating and competitive environment. By taking an ecological perspective and tracking the meme-text from 352 popular memes over the entirety of Reddit, we are able to show that the frequency of memes has scaled almost exactly with the total amount of content created over the past decade. This means that as more data is posted, an equal proportion of memes are posted. One consequence of limited human attention in the face of a growing number of memes is that the diversity of these memes has decreased at the community level, albeit slightly, in the same period. Another consequence is that the average lifespan of a meme has decreased dramatically, which is further evidence of an increase in competition and a decreasing collective attention span.

==> old_notes.tex <==
% another thought here - are we also interested in lifespan as it relates to fraction of uses, instead of fraction of time? are the memes actually experiencing a higher frequency, or is the time just compressed?

% memes are cycling faster - are they peaking higher?

\subsection{other methodology things}

Memes, by definition, have passed some litmus test for transmissibility. And all phrases that fail to become memes are the control group. 

\begin{itemize}
    \item Show the analogues between memes and species, subreddits and communities, adaptations and meme morphings, etc. 
    \item discuss established ecological practices and tools that can readily be applied to the meme space
    \item discuss validation techniques and other junk
\end{itemize}


** 
Within the ecological perspective, there are multiple foci one could consider: the ecosystem as a whole, geographical communities, biome communities, species level communities, right down to individual species. At each of these levels, there are intuitions to be gained.

ecosystem = reddit 
geographical communities = subreddits
biome communities = supposed purpose level similarity of subreddits
species communities = meme similarity derived communities


\subsection{some subreddit-specific analysis}

\begin{itemize}

    \item Meme Richness: Each subreddit has a meme richness measure, which is just the total number of memes that the subreddit has supported at a single time. We can make this value a proportion of the total number of memes that we are investigating to make a value between 0 and 1.
    \begin{itemize}
        \item What does that meme richness look like over time? 
        \item Does the average meme richness increase for subreddits? 
        \item Is the increase linear, or something else?
        \item Is there a seeming upper bound to richness?
    \end{itemize}
    
\iffalse
    \begin{figure}
        \centering
        \includegraphics[width=0.4\textwidth]{tempimages/memerichness.png}
        \caption{average subreddit meme richness over time - should be pretty stable when normalized by reddit growth}
        \label{fig:meme_richness}
    \end{figure}
    
    \begin{figure*}
        \centering
        \subfloat[activity distribution]{\includegraphics[width=0.4\textwidth]{tempimages/activity_hist.png}\label{fig:activity_hist}}
        \hfill
        \subfloat[meme usage]{\includegraphics[width=0.4\textwidth]{tempimages/meme_occurrences.png}\label{fig:meme_occurrences}}
        \hfill
        \subfloat[unique memes]{\includegraphics[width=0.4\textwidth]{tempimages/unique_memes.png}\label{fig:unique_memes_dist}}
        \hfill
        \subfloat[scatter]{\includegraphics[width=0.4\textwidth]{tempimages/subreddit_meme_scatter.png}\label{fig:subreddit_memes}}
        \caption{(a) number of meme occurrences vs number of subreddits, (b) number of unique memes (meme richness) vs number of subreddits, and (c) unique memes (meme richness) vs meme occurrences per subreddit; more unique memes in a subreddit does not necessarily guarantee more meme occurrences}
        \label{fig:memes_over_time}
    \end{figure*}
\fi
    
    \item Meme Evenness: Each subreddit has a meme evenness measure that indicates whether the memes that are contained within the community have relative equality in terms of user usage within the community. This value is inherently between 0 and 1.
    \begin{itemize}
        \item What does this evenness look like over time? Increasing, decreasing, static?
        \item Do certain subreddits have very different evenness values?
    \end{itemize}
    
    \item Meme Diversity: Taking into consideration both meme richness and meme evenness, we can look at the overall meme diversity of a subreddit with respect to time. We can also extend this concept farther, to encompass the entirety of Reddit over time. 
    
\end{itemize}


\cite{le2014distributed}

\section{How to count memes}

% \input{plots/all_ngrams_normed_meme_freq}

\section{How to measure/compare memes}

\begin{itemize}
    \item draw random background phrases of each n-gram length
    \item trace background phrases across all of reddit - frequency per day
    \item to get normalized meme frequency, divide by corresponding n-gram background
\end{itemize}

\begin{figure}
    \centering
    \includegraphics[width=0.4\textwidth]{tempimages/aggregatememe}
    \caption{Sum of all meme frequencies, plotted against 1-gram background}
    \label{fig:aggregate_meme}
\end{figure}


\section{Meme creation is constant}

\section{Meme diversity}\label{sec:meme_diversity}

% \input{plots/all_diversity_avgs}

\section{Invasive Species -- Beachheads}

\section{Discussion}

\begin{itemize}
    \item discuss what it means for memes or subreddits to be diverse
    \item what it means for the level of meming to seem consistent.
    \item 
\end{itemize}
